Privacy-Preserving Database Fingerprinting

When sharing sensitive relational databases with other parties, a database owner aims to (i) have privacy guarantees for the database entries, (ii) have liability guarantees (via fingerprinting) in case of unauthorized sharing of its database by the recipients, and (iii) provide a high quality (utility) database to the recipients. We observe that sharing a relational database with privacy and liability guarantees are orthogonal objectives. The former can be achieved by injecting noise into the database to prevent inference of the original data values, whereas, the latter can be achieved by hiding unique marks inside the database to trace malicious parties (data recipients) who redistribute the data without the authorization. We achieve these two objectives simultaneously by proposing a novel entry-level differentially-private fingerprinting mechanism for relational databases. At a high level, the proposed mechanism fulfills the privacy and liability requirements by leveraging the randomization nature that is intrinsic to fingerprinting and achieves desired entry-level privacy guarantees. To be more specific, we devise a bit-level random response scheme to achieve differential privacy guarantee for arbitrary data entries when sharing the entire database, and then, based on this, we develop an $\epsilon$-entry-level differentially-private fingerprinting mechanism. Next, we theoretically analyze the relationships between privacy guarantee, fingerprint robustness, and database utility by deriving closed form expressions. The outcome of this analysis allows us to bound the privacy leakage caused by attribute inference attack and characterize the privacy-utility coupling and privacy-fingerprint robustness coupling. Furthermore, we also propose a SVT-based solution to control the cumulative privacy loss when fingerprinted copies of a database are shared with multiple recipients.

==> sections/multiple_query.tex <==


\section{Releasing Multiple Fingerprinted Database}\label{sec:multiple_sharing}


One of the major challenges in practical differential privacy is that the data privacy  will degrade if the same statistics are repeatedly calculated and released using the same differentially private mechanism.   The same is true for sharing   a database with multiple SPs. For example, if there are multiple leakage of fingerprinted databases, the average of these copies many eventually converge to the original database, which implies that  the strength of the privacy guarantee of Algorithm \ref{algo:fingerprint_sp_n} degrades with repeated uses. 


However, in practice, the database owner   only releases her database to limited number of SPs, and for each released copy, she   will have certain privacy and fingerprint robustness  requirements. According to Figure \ref{fig:relationships},  the   requirements can both be fulfilled if the utility of the shared database is below a certain level; the error of the shared database is higher than a threshold, which   can be characterized by fingerprint density defined as follows. 

 

% From the previous section we know that the database owner can achieve certain level of differential privacy and fingerprint  robustness by allowing some error in the fingerprinted databases. 



% \begin{definition} 
% A fingerprinted relational database $\mathcal{M}(\R)$ is said to be $\Gamma$-density if $||\mathcal{M}(\R) - \R||_F \geq \Gamma$.
% % \begin{equation}
% %     ||\mathcal{M}(\R) - \R||_F \geq \Gamma.
% %     \label{eq:gamma_density}
% % \end{equation}
% % \label{def:gamma_density}
% \end{definition}


\begin{definition} 
A fingerprinted relational database $\mathcal{M}(\R)$ is said to be $\Gamma$-density if $\mathcal{M}(\R) \ominus \R \geq \Gamma$, where $\ominus$ denotes the symmetric difference that counts the number of different entries between $\mathcal{M}(\R)$ and $\R$.
% \begin{equation}
%     ||\mathcal{M}(\R) - \R||_F \geq \Gamma.
%     \label{eq:gamma_density}
% \end{equation}
% \label{def:gamma_density}
\end{definition}


Therefore, it inspires us to address the problem of privacy degradation under multiple sharing by adopting the sparse vector technique (SVT) \cite{dwork2014algorithmic,lyu2017understanding}. In particular, SVT takes as input a sequence of (potentially adaptive) queries with bounded sensitivity against a fixed database, and returns a sequence of $\bot$ and $\top$, which, respectively, indicate that the result of the corresponding query is below and above a threshold. The unique benefit of SVT is that it can answer multiple queries  while paying the cost of privacy only for the query results  that pass a predefined
threshold, i.e., when the output results are $\top$. In our scenario, the database owner will only have privacy loss if the fingerprint density is above a predetermined value. In the following sections, we first present an intermediate step which releases fingerprint density indicators in a differentially private manner, and then provide the scheme that replaces instances of $\top$ to the actual numerical fingerprinted  databases. 

% The value of $\Gamma$ is determined by the database owner, and we will experimentally investigate its impact on 

\subsection{The Intermediate Step: Releasing Fingerprinting Density Indicator via SVT}



% Theorem \ref{thm:dpfp} suggests that given a privacy budget (i.e., $\epsilon$), 
% % of fingerprinting a database, 
% as long as $p\in[ 1/(e^{\epsilon/K}+1), 0.5)$, the obtained fingerprinted database is $\epsilon$-differentially private.   As a result, there are infinite choices of $p$. To achieve high fingerprinting robustness, we will consider $p$ that can lead to a particular fingerprinting density. In particular, we have the following definition. 

In Section \ref{sec:an_instant}, we have discussed how to generate a differentially private fingerprinted database for a specific SP. Now, we describe the intermediate step that releases, in a privacy-preserving manner,  the above density threshold indicator ($\top$) only one time when there is a sequence of SPs querying the database. 





% determines if the fingerprinted database for each SP $i$ is $\Gamma$-density, and releases the indicators (e.g., $\bot$ and $\top$) in a privacy-preserving manner. 

We summarize the immediate step in Algorithm \ref{algo:FingerprintDensityThresholding}. Specifically, we consider a sequence of ordered SPs with serial number in $\{1,2,3,\cdots\}$. When the $i$th SP queries the database, the database owner first generates a fingerprinted database $\mathcal{M}(\R)$ by applying Algorithm \ref{algo:fingerprint_sp_n} with some privacy budget $\epsilon_1$. Then, she  compares $||\mathcal{M}(\R)-\R||_F$ with a new noisy threshold $\hat{\Gamma}$, which is obtained by perturbing $\Gamma$ with Laplace noise (i.e., $\rho\sim\mathrm{Lap}(\frac{2\Delta}{\epsilon_2/2})$). She will output $a_i=\top$ and terminate the algorithm if $||\mathcal{M}(\R)-\R||_F$ is larger than the noisy threshold, otherwise she will continuously   $a_i=\bot$. 


.  When Algorithm \ref{algo:FingerprintDensityThresholding} halts, we know that the last instance of $\mathcal{M}(\R)$ is higher than $\hat{\Gamma}$ when the last SP queries. The entire process is differentially private, and is proved in the following theorem. 


\begin{algorithm}
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\caption{FingerprintDensityThresholding}\label{algo:FingerprintDensityThresholding}
\Input{Original database $\R$, fingerprinting scheme $\mathcal{M}$, serial number of different SPs, i.e., $\{1,2,3,\cdots\}$, fingerprinting density  threshold $T$, and privacy budget $\epsilon_2$.} % maintained by the data curator.}
\Output{$\{\bot,\bot,\cdots,\bot,\top\}$.}% released to the data consumer.}


\ForAll{$i\in\{1,2,3,\cdots\}$}{

Let $\hat{\Gamma} = \Gamma + \rho$, where $\rho\sim\mathrm{Lap}(\frac{2\Delta}{\epsilon_2/2})$.\label{line:generate_rho} %\algorithmiccomment{get noisy threshold}

Generate   $\mathcal{M}(\R)$ for the $i$th SP using Algorithm \ref{algo:fingerprint_sp_n}.

\eIf{$||\mathcal{M}(\R)-\R||_F \geq \hat{\Gamma}$}{Output $a_i = \top$.

\textbf{Halt}.
}{Output $a_i = \bot$.}
}
\end{algorithm}



\begin{theorem}
Algorithm \ref{algo:FingerprintDensityThresholding} is $\epsilon_1$-deferentially private.
\end{theorem}
\begin{proof}[Proof]  
Suppose that  Algorithm \ref{algo:FingerprintDensityThresholding}  terminates with $l$ outputs, i.e., $\mathbf{a} = [a_1,a_2,\cdots,a_l] = \{\bot\}^{l-1}\cup \{\top\}$. 
% Define $\mathbf{S}_{\top} = \{i:a_i = \top\}$, and $\mathbf{S}_{\bot} = \{i:a_i = \bot\}$. 
By defining   
\begin{equation}
    \begin{aligned}
        &f_i(\R,z) = \Pr(||\mathcal{M}_i(\R)-\R||_F < \Gamma+z),\\
         &g_i(\R,z) = \Pr(||\mathcal{M}_i(\R)-\R||_F  \geq \Gamma+z),
    \end{aligned}
\end{equation}
where $z$ is an instance of $\rho$ generated from Line \ref{line:generate_rho} in Algorithm \ref{algo:FingerprintDensityThresholding},  we   have
\begin{equation*}
    \begin{aligned}
        &\frac{\Pr\Big(\mathrm{FingerprintDensityThresholding}(\R) = \mathbf{a}\Big)}{\Pr\Big(\mathrm{FingerprintDensityThresholding}(\R') = \mathbf{a}\Big)}\\
         =& \frac{\int_{-\infty}^{\infty}\Pr(\rho=z)\prod_{i=1}^{l-1}f_i(\R,z) g_l(\R,z)dz}{\int_{-\infty}^{\infty}\Pr(\rho=z)\prod_{i=1}^{l-1}f_i(\R',z) g_l(\R',z)dz} \\
         \stackrel{(*)}=& \frac{\int_{-\infty}^{\infty}\Pr(\rho=z-2\Delta)\prod_{i=1}^{l-1}f_i(\R,z-2\Delta) g_l(\R,z-2\Delta)dz}{\int_{-\infty}^{\infty}\Pr(\rho=z)\prod_{i=1}^{l-1}f_i(\R',z) g_l(\R',z)dz} = \clubsuit,%\scriptstyle\bigLozenge,
    \end{aligned}
\end{equation*}
where $(*)$ is obtained by  a change of integration variable of $z$ to $z-2\Delta$. Next, we investigate the three parts of the integrand in the numerator of $\clubsuit$ separately. 

First, we have $\Pr(\rho = z-2\Delta)\leq e^{\epsilon_1/2} \Pr(\rho=z)$, as $\rho$ is attributed to a Laplace distribution whose parameter is calibrated using $2\Delta$. 

Second, since $||\mathcal{M}_i(\R')-\R'||_F - ||\mathcal{M}_i(\R)-\R||_F \leq ||\mathcal{M}_i(\R')-\R'-\mathcal{M}_i(\R)+\R||_F\leq ||\mathcal{M}(\R')-\mathcal{M}(\R)||_F+||\R'-\R||_F\leq2\Delta$, where the last inequality is due to the  sensitivity-invariant property in (\ref{eq:invariant}), thus, $||\mathcal{M}_i(\R')-\R'||_F\leq ||\mathcal{M}_i(\R)-\R||_F+2\Delta$. As a result, we obtain $f_i(\R,z-2\Delta) =$ 
\resizebox{1\hsize}{!}{$\Pr\Big(||\mathcal{M}_i(\R)-\R||_F + 2\Delta< \Gamma+z\Big) \leq \Pr\Big(||\mathcal{M}_i(\R')-\R'||_F  < \Gamma+z\Big)=$} $f_i(\R',z)$. 




Third, following the same analysis of the first part, we have $g_l(\R,z-2\Delta) = \Pr\Big(||\mathcal{M}_i(\R)-\R||_F+2\Delta  \geq \Gamma+z\Big)\leq e^{\epsilon_1/2}\Pr\Big(||\mathcal{M}_i(\R')-\R'||_F   \geq \Gamma+z\Big)  = e^{\epsilon_1/2} g_l(\R',z)$. As a result, we have 
\begin{equation*}%\begin{aligned}
        \clubsuit\leq \frac{\int_{-\infty}^{\infty}e^{\epsilon_1/2} \Pr(\rho=z)\prod_{i=1}^{l-1}f_i(\R',z)  e^{\epsilon_1/2} g_l(\R',z)dz}{\int_{-\infty}^{\infty}\Pr(\rho=z)\prod_{i=1}^{l-1}f_i(\R',z) g_l(\R',z)dz}   = e^{\epsilon_1},
% \end{aligned}
\end{equation*}
which concludes the proof.
\end{proof}


\subsection{Composition of   Intermediate Steps: Releasing Multiple Numerical Fingerprinted Databases}

Now, we can arrive at Algorithm \ref{algo:MultipleFingerprintedDatabasesReleasing}, which     outputs the numeric fingerprinted databases that are above the noisy thresholds for various SPs. Suppose that the database owner will only share her  fingerprinted databases with at most $C$ SPs. For the $i$th SP, it will receive the fingerprinted database, i.e., $\top$ is replaced with $\mathcal{M}(\R)$, if $||\mathcal{M}(\R)-\R||_F \geq \hat{\Gamma}$, where $\mathcal{M}(\R)$ is generated by adopting Algorithm \ref{algo:fingerprint_sp_n} with privacy budget $\epsilon_2' = \frac{\epsilon_2}{\sqrt{8c\ln(\frac{2}{\delta})}}$, and $\hat{\Gamma}$ is obtained from the Laplace mechanism with privacy budget $\epsilon_1' = \frac{\epsilon_1}{\sqrt{8c\ln(\frac{2}{\delta})}}$. Otherwise, the database owner will not share the $i$th SP.




% In particular, 

\begin{algorithm}
\small
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\caption{MultipleFingerprintedDatabasesReleasing}\label{algo:MultipleFingerprintedDatabasesReleasing}
\Input{Original database $\R$, fingerprinting scheme $\mathcal{M}$, the Bernoulli distribution parameter  $p\geq \frac{1}{e^{\epsilon/K}+1}$,  serial number of different SPs, i.e., $\{1,2,3,\cdots\}$, fingerprinting density  threshold $\Gamma$, and privacy budget $\epsilon_1$, $\epsilon_2$, and $\delta$.} % maintained by the data curator.}
\Output{$\{a_1,a_2,a_3,\cdots\}$.}% released to the data consumer.}


Set   $\epsilon_1' = \frac{\epsilon_1}{\sqrt{8c\ln(\frac{2}{\delta})}}$, $\epsilon_2' = \frac{\epsilon_2}{\sqrt{8c\ln(\frac{2}{\delta})}}$, and $count=0$.

% Set $p_{\mathrm{row}} = 1-\prod_{t=1}^{|\mathcal{T}|}(1-p)^{K_t}$;


\ForAll{$i\in\{1,2,3,\cdots\}$}{

% Initiate $p=p_0$.


Let $\hat{\Gamma} = \Gamma + \rho$, where $\rho\sim\mathrm{Lap}(\frac{2\Delta}{\epsilon_1'/2})$. %\algorithmiccomment{get noisy threshold}\label{line:generate_rho}



% \While{$count<C$}{

Obtain $\mathcal{M}(\R)$ by applying algorithm \ref{algo:fingerprint_sp_n}   with privacy budget $\epsilon_2'$ and probability $p$.


\eIf{$||\mathcal{M}(\R)-\R||_F \geq \hat{\Gamma}$}{

Output $a_i=\mathcal{M}(\R)$. \algorithmiccomment{the $i$th SP receives the fingerprinted database.}

% Set $p_{\mathrm{row}} = 1-\prod_{t=1}^{|\mathcal{T}|}(1-p)^{K_t}$;

$count=count+1$.

\If{$count==C$}{
\textbf{Halt}.}
}{

% Update $p=p+\frac{1}{NKT}$;

Output $a_i = \bot$.\algorithmiccomment{the $i$th SP done not receive the fingerprinted database.}

}
% }


}




\end{algorithm}




\begin{theorem}
Algorithm \ref{algo:MultipleFingerprintedDatabasesReleasing} is ($\epsilon_1+\epsilon_2,\delta$)-deferentially private.
\end{theorem}
\begin{proof}[Proof]  
Algorithm \ref{algo:MultipleFingerprintedDatabasesReleasing} is the composition of $C$ rounds of Algorithm   \ref{algo:FingerprintDensityThresholding} with $C$ rounds of Algorithm   \ref{algo:fingerprint_sp_n}. According to the Advanced Composition theorem (p. 49 \cite{dwork2014algorithmic}), $C$ rounds of Algorithm   \ref{algo:FingerprintDensityThresholding} and $C$ rounds of Algorithm   \ref{algo:fingerprint_sp_n} are $(\epsilon_1,\delta/2$)-deferentially private and $(\epsilon_2,\delta/2$)-deferentially private, respectively. Then, by simple composition of those two, we complete the proof.
\end{proof}

==> sections/threat_models.tex <==


\section{Threat Models}
\label{sec:threat_models}

\subsection{Membership Inference Attack}
can we  prevent membership inference attacks?

If we add controlled noise to the database, we will keep the noise limited to make sure we dont lose too much utility (just consider your XOR mechanism for simplicity). If the attacker already has the entire (genomic) data of a victim, then the attacker can just compute the edit or Hamming distance between the victim's genome and all genomes in the received dataset and based on this edit distance, the attacker cn infer the membership of the victim to the shared dataset. DP (at least the way we use it to share databases)  






% \subsection{Fingerprint Robustness Metrics}




% \subsection{Database Utility Metrics}
